Cherenkov Telescope Array sensitivity to the putative millisecond pulsar population responsible for the Galactic center excess

The leading explanation of the $\textit{Fermi}$ Galactic center $\gamma$-ray excess is the extended emission from a unresolved population of millisecond pulsars (MSPs) in the Galactic bulge. Such a population would, along with the prompt $\gamma$ rays, also inject large quantities of electrons/positrons ($e^\pm$) into the interstellar medium. These $e^\pm$ could potentially inverse-Compton (IC) scatter ambient photons into $\gamma$ rays that fall within the sensitivity range of the upcoming Cherenkov Telescope Array (CTA). In this article, we examine the detection potential of CTA to this signature by making a realistic estimation of the systematic uncertainties on the Galactic diffuse emission model at TeV-scale $\gamma$-ray energies. We forecast that, in the event that $e^\pm$ injection spectra are harder than $E^{-2}$, CTA has the potential to robustly discover the IC signature of a putative Galactic bulge MSP population sufficient to explain the GCE for $e^\pm$ injection efficiencies in the range $\approx 2.9-74.1\%$, or higher, depending on the level of mismodeling of the Galactic diffuse emission components. On the other hand, for spectra softer than $E^{-2.5}$, a reliable CTA detection would require an unphysically large $e^\pm$ injection efficiency of $\gtrsim 158\%$. However, even this pessimistic conclusion may be avoided in the plausible event that MSP observational and/or modeling uncertainties can be reduced. We further find that, in the event that an IC signal were detected, CTA can successfully discriminate between an MSP and a dark matter origin for the radiating $e^\pm$.

==> gitignore <==
main.pdf
# Created by https://www.gitignore.io/api/tex,latex,emacs
# Edit at https://www.gitignore.io/?templates=tex,latex,emacs

### Emacs ###
# -*- mode: gitignore; -*-
*~
\#*\#
/.emacs.desktop
/.emacs.desktop.lock
*.elc
auto-save-list
tramp
.\#*

# Org-mode
.org-id-locations
*_archive

# flymake-mode
*_flymake.*

# eshell files
/eshell/history
/eshell/lastdir

# elpa packages
/elpa/

# reftex files
*.rel

# AUCTeX auto folder
/auto/

# cask packages
.cask/
dist/

# Flycheck
flycheck_*.el

# server auth directory
/server/

# projectiles files
.projectile

# directory configuration
.dir-locals.el

# network security
/network-security.data


### LaTeX ###
## Core latex/pdflatex auxiliary files:
*.aux
*.lof
*.log
*.lot
*.fls
*.out
*.toc
*.fmt
*.fot
*.cb
*.cb2
.*.lb

## Intermediate documents:
*.dvi
*.xdv
*-converted-to.*
# these rules might exclude image files for figures etc.
# *.ps
# *.eps
main.pdf

## Generated if empty string is given at "Please type another file name for output:"
.pdf

## Bibliography auxiliary files (bibtex/biblatex/biber):
*.bbl
*.bcf
*.blg
*-blx.aux
*-blx.bib
*.run.xml

## Build tool auxiliary files:
*.fdb_latexmk
*.synctex
*.synctex(busy)
*.synctex.gz
*.synctex.gz(busy)
*.pdfsync

## Build tool directories for auxiliary files
# latexrun
latex.out/

## Auxiliary and intermediate files from other packages:
# algorithms
*.alg
*.loa

# achemso
acs-*.bib

# amsthm
*.thm

# beamer
*.nav
*.pre
*.snm
*.vrb

# changes
*.soc

# comment
*.cut

# cprotect
*.cpt

# elsarticle (documentclass of Elsevier journals)
*.spl

# endnotes
*.ent

# fixme
*.lox

# feynmf/feynmp
*.mf
*.mp
*.t[1-9]
*.t[1-9][0-9]
*.tfm

#(r)(e)ledmac/(r)(e)ledpar
*.end
*.?end
*.[1-9]
*.[1-9][0-9]
*.[1-9][0-9][0-9]
*.[1-9]R
*.[1-9][0-9]R
*.[1-9][0-9][0-9]R
*.eledsec[1-9]
*.eledsec[1-9]R
*.eledsec[1-9][0-9]
*.eledsec[1-9][0-9]R
*.eledsec[1-9][0-9][0-9]
*.eledsec[1-9][0-9][0-9]R

# glossaries
*.acn
*.acr
*.glg
*.glo
*.gls
*.glsdefs

# uncomment this for glossaries-extra (will ignore makeindex's style files!)
# *.ist

# gnuplottex
*-gnuplottex-*

# gregoriotex
*.gaux
*.gtex

# htlatex
*.4ct
*.4tc
*.idv
*.lg
*.trc
*.xref

# hyperref
*.brf

# knitr
*-concordance.tex
# TODO Comment the next line if you want to keep your tikz graphics files
*.tikz
*-tikzDictionary

# listings
*.lol

# luatexja-ruby
*.ltjruby

# makeidx
*.idx
*.ilg
*.ind

# minitoc
*.maf
*.mlf
*.mlt
*.mtc[0-9]*
*.slf[0-9]*
*.slt[0-9]*
*.stc[0-9]*

# minted
_minted*
*.pyg

# morewrites
*.mw

# nomencl
*.nlg
*.nlo
*.nls

# pax
*.pax

# pdfpcnotes
*.pdfpc

# sagetex
*.sagetex.sage
*.sagetex.py
*.sagetex.scmd

# scrwfile
*.wrt

# sympy
*.sout
*.sympy
sympy-plots-for-*.tex/

# pdfcomment
*.upa
*.upb

# pythontex
*.pytxcode
pythontex-files-*/

# tcolorbox
*.listing

# thmtools
*.loe

# TikZ & PGF
*.dpth
*.md5
*.auxlock

# todonotes
*.tdo

# vhistory
*.hst
*.ver

# easy-todo
*.lod

# xcolor
*.xcp

# xmpincl
*.xmpi

# xindy
*.xdy

# xypic precompiled matrices
*.xyc

# endfloat
*.ttt
*.fff

# Latexian
TSWLatexianTemp*

## Editors:
# WinEdt
*.bak
*.sav

# Texpad
.texpadtmp

# LyX
*.lyx~

# Kile
*.backup

# KBibTeX
*~[0-9]*

# auto folder when using emacs and auctex
./auto/*
*.el

# expex forward references with \gathertags
*-tags.tex

# standalone packages
*.sta

### LaTeX Patch ###
# glossaries
*.glstex

### TeX ###

# these rules might exclude image files for figures etc.
# *.ps
# *.eps
# *.pdf




# latexrun

# algorithms

# achemso

# amsthm

# beamer

# changes

# comment

# cprotect

# elsarticle (documentclass of Elsevier journals)

# endnotes

# fixme

# feynmf/feynmp


# glossaries

# uncomment this for glossaries-extra (will ignore makeindex's style files!)
# *.ist

# gnuplottex

# gregoriotex

# htlatex

# hyperref

# knitr
# TODO Comment the next line if you want to keep your tikz graphics files

# listings

# luatexja-ruby

# makeidx

# minitoc

# minted

# morewrites

# nomencl

# pax

# pdfpcnotes

# sagetex

# scrwfile

# sympy

# pdfcomment

# pythontex

# tcolorbox

# thmtools

# TikZ & PGF

# todonotes

# vhistory

# easy-todo

# xcolor

# xmpincl

# xindy

# xypic precompiled matrices

# endfloat

# Latexian

# WinEdt

# Texpad

# LyX

# Kile

# KBibTeX

# auto folder when using emacs and auctex

# expex forward references with \gathertags

# standalone packages

### TeX Patch ###
# glossaries

# End of https://www.gitignore.io/api/tex,latex,emacs

